Contact Angle Hysteresis on Rough Surfaces Part I: Mechanical Energy Balance Framework

Using as a starting point conservation of momentum, a multiphase mechanical energy balance equation is derived that accounts for multiple material phases and interfaces present within a moving control volume. This balance is applied to a control volume that is anchored to a three phase contact line as it advances over the surface of a rough and chemically homogeneous solid. Using semi-quantitative models for the material behaviour occurring within the control volume, an order-of-magnitude analysis is performed to find what terms within the balance are significant, producing an equation that can be used to predict contact angle hysteresis from a knowledge of interface dynamics occurring around the three phase contact line. In addition to this equation, the theory also answers several questions that have been discussed within the wetting literature: Namely that (static) contact angle hysteresis is a function of conditions around the three phase contact line, as opposed to the surrounding flow system; That contact angle hysteresis results from interface `jumps' that dissipate energy, rather than directly from contact line deformation; That interfacial dynamics is required to predict contact angle hysteresis, but that these dynamics should be interpreted via energy conservation, and; That dynamic contact angles depend on kinetic energy transport around the three phase contact line, as well as local energy dissipation. The framework has been derived using assumptions of incompressible Newtonian fluids, reversible interface formation and zero-strain solids -- future work could relax these assumptions to make the theory more generally applicable.

==> junk.tex <==

\newpage


Broadly speaking, energetic theories employ an energy balance over some defined volume to predict contact angle hysteresis.

Existing theories concerned with wetting on rough surfaces are either kinetically or energetically based.  Kinetically based theories employ a force balance.  \Citet{cox83} solved Laplace's equation to show how the `macroscopic contact angle' varied as an interface moved over a surface having periodic and sinusoidal roughness.  While the kinetic analysis was certainly rigorous in predicting interface topologies as a function of interface displacement and angle (given the small solid gradient assumption), it was assumed that the variation of the macroscopic contact angle represented contact angle hysteresis. This assumption is at odds with the definition of contact angle hysteresis however which is not concerned with the variation in contact angle during a continuous (eg) advance of the interface, but rather the variation between the static advancing and receding angles. While \Citeauthor{cox83} did explore other interpretations of the analysis, the theory does not directly link the range of macroscopic static contact angles to id not directly link did calculate energy dissipation due to interfacial jumps, but this was not the focus of the study.  Kinetically based theories for anisotropic roughness do not capture wetting behaviour observed on real, isotropic surfaces~\citep{johnson64,brandon03}.

\citep{brandon03} is concerned with finding equilibrium angle using surface evolver on periodic rough surfaces.  The greater the drop to roughness ratio, the closer the minimum droplet energy approaches the Cassie angle.  Simultaneously the 


Energetic modelling that includes dissipation (leading to contact angle hysteresis) has been explored previously, but not in the context of the rough and random multiscale surfaces considered here.  \Citet{joanny84} proposed a model for contact angle hysteresis on a surface that contains a dilute number of `strong defects' --- a model for surface contamination.  Hysteresis was predicted in terms of the geometry of the deformed interface.  The model was extended to surface roughness, but only (quantitatively) for regular, rectangular defects.  Recently, in interpreting the movement of liquids over regular arrays of rectangular holes and poles in the Wenzel and fakir states, Ralston's group has found that the normalised energy dissipation per interface structure (defect) is roughly independent of structure density, provided that the wetting state is known \citep{priest09,forsberg10}.  This observation is consistent with the present modelling approach.  In a comprehensive recent review of the field, \citet{ramiasa14} shows that hysteresis scaling arguments have been successfully employed (notably in the 1980's and 1990's) in several idealised limits (e.g., strong pinning and low density, weak pinning and high density defects), but that no group has used the theory to develop a quantitative wetting model for significantly sized deflects.  \textbf{One reason why such a theory has not been developed is that the modelling technology capable of capturing the interface deformation and fluid flow on the lengthscale of the surface roughness has previously not been available to those in the field.}

%Note that since \citeauthor{barthlott97}'s inspiring work on the self-cleaning lotus leaf was published in the late 1990s, there has been a tremendous amount of research conducted into superhydrophobic surfaces.  Indeed, a 2011 global research citation report ranked `superhydrophobic surfaces' as seventh amoung 438 current research activities within chemistry, physics, engineering and biological sciences\citep{wen15}.  While this activity does hint at the benefits of `smarter' wetting, the research of is limited use in our analysis of `real', hierarchically rough surfaces.  The idealised superhydrophobic surfaces are typically composed of periodically arranged and regularly shaped poles made via photolithography, which have a single lengthscale, display anisotropic wetting and most importantly, are densely spaced flat topped structures which bear little resemblance to the roughness found on most engineering and natural surfaces.  In this project super-wetting surfaces (a term which captures all of the extreme wetting states, such as superhydrophobic, superhydrophilic, superoleophobic, superaerophobicity, etc\cite{wen15}) will not be the focus --- intermediately wetting surfaces are the most important for model validation, and are also the most sparsely considered in the literature.

\subsection{Aim}

  Our aim is to predict these two angles for a randomly structured, chemically homogeneous surface that has multiple roughness lengthscales.  Note that this study is not concerned with dynamic contact angles (the angle measured during liquid flow over a surface).

The purpose of this paper is to explain the phenomenon of contact angle hysteresis in terms of microbubble formation and relaxation.   In this context `microbubble' describes any small packet of fluid which exists within the depressions of the rough solid surface, but is bounded above by another fluid with which it is immiscible.  After formulating the problem in general terms, we propose a simple model for the kinetics of a bubble which is formed and relaxes on a saw tooth surface.  We use this model to find advancing and receding angles on both dry and wet surfaces in terms of the `Youngs' equilibrium angle and two solid roughness parameters.  Predictions from the model reproduce some fundamental experimental observations, reinforcing the postulate that rough solid contact angle hysteresis is a macroscopic manifestation of microbubble kinetics.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%A liquid wetting a solid is a ubiquitous process that occurs in a wide variety of natural, industrial and domestic processes.  Recent studies are finding that in nature, organisms use specific surface structures to control wetting behaviour, to the advantage of the organism.  Researchers are trying to replicate such functionalised wettability, using microengineered surfaces.  What hampers these efforts however is a lack of theory linking surface morphology to surface wettability.  The ARF applicant has recently proposed such a theory.  The aim of this Discovery Project is to validate and extend this theory, not only to provide a tool to allow functionalised surface design, but also to increase our understanding of the physical processes that occur when a liquid wets a real surface.  The project will support the ARF applicant, and two PhD students.

The ability of a liquid to `wet' a solid is described by the angle that the liquid makes with the solid when the system is in equilibrium --- the contact angle.  If a liquid wets a solid well, then the contact angle is low.  If it wets a solid poorly, then the contact angle is high.  For a droplet resting on a smooth and chemically homogeneous (chemically uniform) surface, the contact angle, $\scal[e]{\theta}$, is given by Young's Equation (see equation in figure \ref{fig:wetting_states}a).  When the angle the liquid makes with the solid is greater than $\scal[e]{\theta}$, the liquid advances;  when the angle is less, the liquid recedes.  Real surfaces, which are often rough on length scales that are small relative to that of the surrounding flow, or have a chemical composition which varies with location (chemically heterogeneous), display a range of contact angles within which a liquid interface can remain stationary.  For these surfaces the equilibrium contact angle range is specified by an upper bound, the advancing angle $\scal[a]{\theta}$, and by a lower bound, the receding angle, $\scal[r]{\theta}$.   The advancing and receding angles measured on real surfaces may be far removed from Young's angle, $\scal[e]{\theta}$.  Further, the difference between the two angles, the hysteresis, may be large.

%These surfaces interact with their environment to the advantage of the organism.  

\begin{figure}[htbp]
\centering
\resizebox{0.9\textwidth}{!}{\input{demonstration_surfaces.pdf_t}} % fig from xfig that includes latex text
\caption{Functionalised Wettability:  Micro (a) and Nano (b) sized structures on the lotus leaf \citep[from][]{barthlott97,sun05}, superhydrophobic transparent PMMA (c) \citep[from][]{wu02}, anisotropic rice leaf (d) and replica ACNT surface (e) \citep[from][]{sun05} and mesh for oil water separation, structure (f) and performance (g) \citep[from][]{feng04} (Images adapted from references).\label{fig:demonstration_surfaces}}
\end{figure}

Recent studies have shown that in nature, plants and animals use specific surface roughness, often combined with chemical heterogeneity, to produce surfaces with functionalised wettability.  The sacred lotus (figure \ref{fig:demonstration_surfaces}a-b) uses a combination of fine nanostructures ($120 \units{nm}$), micropapillae ($5-9 \units{\mu m}$) and cuticular waxes to produce a leaf that is superhydrophobic --- that is, a surface with a very high advancing contact angle for water~\citep{barthlott97,sun05}.  This superhydrophobicity, combined with low contact angle hysteresis, means that water droplets roll off lotus leaves easily, collecting and removing any debris from the surface as they go.  This keeps the surface of the leaf clean, maximising the efficiency of the plant's photosynthesis.  The self-cleaning `lotus effect' is now recognised in over 200 species of plants \citep{parkin04}, as well as on the wings of insects such as butterflies and cicadae \citep{feng06}.  The rice leaf (figure \ref{fig:demonstration_surfaces}d) possesses anisotropic (directionally dependent) surface structures which causes water to roll preferentially along the length of the leaf, rather than towards its edge \citep{feng02}.  This may aid in cleaning the leaf or collecting water.  The legs of the water strider are so hydrophobic, primarily as a result of the micro and nano sized structures found on the surface of its legs, that it is able to support about 15 times its own weight when standing on water \citep{gao04}.  Even the proverbial rolling of `water off a duck's back' is believed to result from the specific microstructure of the duck's feathers, rather than from any preening oils as was traditionally thought \citep{rijke68}.

%Inspired by the identification of these naturally occurring functionalised surfaces, in particular by the analysis of the lotus effect by \citeauthor{barthlott97} in 1997, a revolution in interface science has begun with researchers racing to design novel surfaces having wettability tailored to meet specific applications.

Inspired by the identification of these naturally occurring functionalised surfaces, a revolution in interface science has begun with researchers racing to design novel surfaces having wettability tailored to meet specific applications.

So far both metallic and polymeric materials have been rendered superhydrophobic and/or anti-fouling by creating micro and nano sized structures on their surfaces.  Techniques such as crystallisation, template synthesis, phase separation, electrochemical deposition, electrospinning and etching have all been used for this process \citep{erbil03,acatay04,yin05,qian05,liu06,artus06,feng06}.  An optically transparent self-cleaning surface (figure \ref{fig:demonstration_surfaces}c) has been created on both glass and polymeric optical substrates \citep{wu02}.  This surface is characterised by surface structures of size less than approximately $100 \units{nm}$, required so that incident light is not scattered by the roughness as it passes into the transparent medium.  If the surface design and manufacturing process used by this technology could be optimised, then the potential application areas for it would be large, spanning fields such as building and automotive glazing, through to photovoltaic cell coverings.

Surfaces with more varied wetting functions have also been produced.  An anisotropically wetting surface (figure \ref{fig:demonstration_surfaces}e) has been constructed using aligned carbon nanotubes (ACNT) \cite{sun03}.  This surface displays directionally dependent wetting behaviour similar to that of the rice leaf, and could find application in Micro-Electro-Mechanical Systems (MEMS) and lab-on-a-chip devices to allow sample transport and manipulation in preferential directions~\citep{shastry06}.  A structured surface coating that is both superhydrophobic and superoleophilic (oil wets the surface well) has been applied to a porous steel mesh (figure \ref{fig:demonstration_surfaces}f-g) to create a simple and robust mechanism capable of separating oil from water \citep{feng04}:  Water applied to the mesh forms beads on its upper surface, remaining mobile to roll tangentially off the mesh and into a catchment reservoir;  Diesel applied to the mesh quickly wets the surface, before falling through.

These innovative surface designs demonstrate the impact that functionalised wettability could have on real world applications.  \textbf{However, no published theory is available that quantifies the link between surface morphology and wetting behaviour.}  This severely limits our ability to perform surface design, and to realise the potential of this emerging research field.

Existing theories describing wetting behaviour on rough surfaces can be broadly classified as either kinetically based, or energetically based.

Kinetically based theories employ a force balance on the liquid/gas interface to determine the macroscopic angle of the advancing interface.  \Citet{shuttleworth48} and \citet{johnson64} developed theories for surfaces with anisotropic roughness (e.g. parallel grooves).  These theories do not capture the behaviour observed on real, isotropic surfaces~\citep{brandon03}.  \Citet{cox83} attempted to resolve the movement of the liquid/gas interface over a gently sloped surface using a rigorous mathematical treatment.  Significantly, he recognised that energy is dissipated whenever the interface has to `jump' from one stable position to another as it advances over local surface undulations, resulting in contact angle hysteresis.  Due to the constrictive assumptions required to make the problem tractable, hysteresis was only predicted when specific sinusoidal forms were assumed for the surface morphology~\citep{cox83}.  De Gennes and coworkers~\citep{joanny84,degennes85}, in their study of interface movement over a surface containing chemical contaminations, also recognised that discrete interface movements result in contact angle hysteresis.

Energetic theories employ an energy balance on a defined volume of liquid to determine whether the liquid/gas interface will advance.  Considering the energy change that occurs as a liquid interface advances a small distance over the surface of a rough solid, \citet{wenzel36} proposed that the cosine of the apparent contact angle increases with the roughness of the surface (see equation in figure \ref{fig:wetting_states}b).  In deriving this theory, \citeauthor{wenzel36} assumed that the liquid completely wets each undulation of the solid (e.g., figure \ref{fig:wetting_states}b for a sawtooth surface).  \Citet{cassie48} recognised that in real systems, such wetting did not necessarily occur, and that the proportion of each undulation that was wetted by the liquid would depend on the morphology of the solid, as well as the manner in which the contact line advanced or receded.  In the extreme case of a liquid wetting only the uppermost surfaces of the solid, a so-called `fakir' droplet, \citet{cassie44} derived an expression for the apparent contact angle (see equation in figure \ref{fig:wetting_states}c for a square wave surface).  This angle is (very approximately) observed for fakir droplets resting on manufactured ultrahydrophobic surfaces, when the surface is composed of periodic structures that have flat upper surfaces \citep{oner00}.

\begin{figure}[htbp]
\center\small\vspace*{1ex}%
\begin{tabular*}{0.9\textwidth}{@{\extracolsep{\fill}}ccc}%
(a) Young's Equilibrium & (b) Wenzel & (c) Fakir %
\\[3ex]%
\resizebox{0.25\textwidth}{!}{\input{young.pdf_t}}% fig from xfig that includes latex text
&%
\resizebox{0.25\textwidth}{!}{\input{wenzel.pdf_t}}% fig from xfig that includes latex text
&%
\resizebox{0.25\textwidth}{!}{\input{cassie.pdf_t}}% fig from xfig that includes latex text
\\[2ex]%
$\cos\scal[e]{\theta}= (\scal[sg]{\sigma}-\scal[ls]{\sigma})/\scal[lg]{\sigma}$%
&%
$\cos\theta = \phi\cos\scal[e]{\theta}$%
&%
$\cos\theta = \scal[ls]{\phi}(\cos\scal[e]{\theta} + 1) - 1$%
\end{tabular*}
\caption{Schematics and equations representing the various wetting states.  In (a), $\scal[lg]{\sigma}$, $\scal[ls]{\sigma}$ and $\scal[sg]{\sigma}$ are the surface energies of the liquid/gas, liquid/solid, and solid/gas interfaces, respectively.  In (b), $\phi$ is the surface area of the rough solid per unit projected area of solid.  In (c), $\scal[ls]{\phi}$ is the surface area along the top of the undulations, per unit projected area of the solid. \label{fig:wetting_states}}
\end{figure}

The Wenzel and fakir states are useful concepts for understanding and interpreting experimental data;  however, theories based solely on these concepts \citep[e.g.][]{shibuichi96,bico02,patankar03} are not predictive.  As has long been recognised~\citep{cassie48}, the proportion of solid surface wetted by a liquid is not known a priori, except for certain idealised systems \citep{quere02}.  Also, these theories give only one `equilibrium' contact angle for a structured surface, rather than a range of stable contact angles as observed on real surfaces \citep{callies05}.  This means that these theories cannot predict the mobility of droplets to move across structured surfaces.

\pagebreak

\begin{floatingfigure}[r]{0.3\textwidth}
\centering
\includegraphics[keepaspectratio,width=0.3\textwidth]{../figures/bartell/bartell53_fig1.png}
\caption{Model paraffin surfaces used by Bartell and coworkers.  Pyramid base dimensions were varied between $250\units{\mu m}$ and $750\units{\mu m}$. \label{fig:bartell_surface}}
\end{floatingfigure}

In a particularly insightful series of papers, Bartell and coworkers~\citep{shepard53,bartell53,bartell53b} used well defined paraffin surfaces textured with micron sized pyramid structures (see figure \ref{fig:bartell_surface}) to study the relationship between contact angle hysteresis, surface morphology and Young's equilibrium angle.  Interestingly, when the surface structures were small relative to the droplet size, macroscopic contact angles were determined by the form (geometry) of the surface structures, rather than by their size.  Further, detailed observations were made describing how the liquid/gas interface often `jumped' over individual surface undulations, and how gas microbubbles or liquid microdroplets were often captured between adjacent surface undulations as the interface progressed over the solid.  \Citet{bankoff58} later discussed some of the theoretical implications of these observations.





%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%


A liquid wetting a solid is a universal process that occurs in a wide variety of natural, industrial and domestic systems.  Recent studies are finding that in nature, organisms use specific surface structures to control wetting, to the advantage of the organism.  Researchers are trying to replicate such functionalised wettability, using microengineered surfaces.  What hampers these efforts though is a lack of theory linking surface morphology to wettability.  The ARF applicant has recently proposed the basis of such a theory.  The aim of this proposal is to develop and validate this theory, not only to provide a tool to allow functionalised surface design, but also to increase our understanding of the physical processes that occur when a liquid wets a real surface.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Theory:}

Early works, looking at energy change with interface movement
\citet{wenzel36} --- both phases completely wetting, but interface area increases
\citet{cassie44} --- builds on wenzel, rough surface, but one phase does not wet surface --- applied to porous surfaces to good effect --- may also describe energy balance at contact line with superhydrophobic surfaces.

\citet{johnson64}

\citet{long05} --- looks at energy change as droplet free energy changes as droplet moves over individual surface oscillations --- These studies predict that contact angle hysteresis should decrease as size of oscillations decreases, as energy barriers to movement become smaller.  These trends are not seen experimentally --- see eg \citet{brandon03}

Similar, related, vein: contact line halted by individual surface topology --- ie, force balance on contact line on uneven surface \citet{shuttleworth48} --- does not match experimental observation, eg, \citet{miller96} study referred to in \citet{long05} study --- different surface `angles' in different directions --- what physical basis???

%\begin{figure}[h]
%\centering%
%\subfigure[\label{fig:dettre64b_fig1}]{\includegraphics[keepaspectratio,width=0.48\textwidth]{./figures/angle_scans/dettre64b_fig1.png}}%
%\subfigure[\label{fig:dettre64b_fig2}]{\includegraphics[keepaspectratio,width=0.48\textwidth]{./figures/angle_scans/dettre64b_fig2.png}}%
%\caption{Water contact angles on TFE-methanol telomer wax surface as a function of roughness (a) and photomicrographs of the same surfaces (b) \citep[taken from][]{dettre64b}.}%
%\label{fig:dettre64b_fig12}%
%\end{figure}

%\subsubsection{Experiments:}

Some do not appreciate difference between advancing on wet and dry surfaces, description somewhat vague.
Limited quantitative data on nature of surface roughness useful for hysteresis prediction, however, some studies give qualitiative description of surface (AFM,ESM etc).
Studies may be complicated by adsorbtion and chemical effects.

\citet{miller96}
\citet{lam01}

\citet{muller01} grew well defined `nanopyramids' on surface, and found that \emph{....contact-angle hysteresis can partly be explained by the barrier effect, which gives rise to symmetric hysteresis, and the capillary effect, which leads to a contact angle reduction, (but) another phenomenon must exist to describe the hysteresis shown in figure 3...} (ALSO, QUESTION THEN, WHAT SCALES DOES THEORY GO DOWN TO?)

%Purpose:  To use a heuristic model of nanobubble formation to simulate contact angle hysteresis.

%\subsection{Purpose}



















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%for the ultimately the surface energy being lost from three interfaces will be converted to heat via viscous dissipation, given that the region of rapid interface movement is confined to small distances from the TPCL.

%water advancing over surfaces having roughnesses of order ..., it is the momentum terms that limit the velocity, giving ...


\newpage


We now impose some constraints on the variables introduced in our model.
To find an order estimate for this velocity, 

constraint on tcap means constraint on n?
%\begin{equation}

%\end{equation}


However as the TPCL is advancing some local areas of the interface may become pinned by surface defects.  When these pinned locations interface 

%for short times within this period the TPCL moves at much faster speeds, driven by capillary forces.  These capillary driven events result in viscous dissipation which has been qualitatively described by \citep


While the speed at which the control volume advances ($\vcv$) is constant, as the gradient of the solid surface varies as a result of the roughness, the speed at which the TPCL advances may change considerably from one location to the next.  However, as the contact line always remains within the control volume, kinematic constraints dictate that \emph{for the majority of the time} the speed at which the contact line moves must be of the same order (or less) as that at which control volume is advancing.  Hence, for the majority of the time the contact line moves at a speed of $\order{\vcv}$.  Noting that this is also the speed that fluid is moving in the surrounding hydrodynamic flow (in an order of magnitude sense), for the majority of the time fluid velocities within control volume will be $\order{\vcv}$ or less everywhere.  We describe the system as being in equilibrium when this is the case.

TODO:
\begin{itemize}
\item precise geometry of interface (why)?
\item vcap
\item times at vacp and vc
\item also stress within fluid, grad v and p
\item stress within solid
\end{itemize}


This study is concerned with contact angle behaviour in the limit of $\vcv\rightarrow0$.  If the system is in equilibrium and we let $\vcv\rightarrow0$, we effectively have a system in which all fluid velocities are zero.  As the fluid interface is bounded by the two fluid phases, it follows that under these conditions the velocity of the interface is also zero, and hence in equilibrium.  

In an order of magnitude sense we can describe the topology of the fluid interface when in equilibrium by examining the system at different lengthscales.  Applying momentum balance equation~(\ref{eq:momentum}) within the volume of each fluid phase and taking the limit as $\abs{\vect{v}}\rightarrow0$ shows that the hydrostatically adjusted pressure, $P=p+\rho \hat{\Phi}$, is uniform within each fluid phase\footnote{Here we have assumed $\tens[M]{T}\rightarrow p\tens{I}$ as $\vect{v}\rightarrow0$.  This property essentially defines a fluid.}.  Further, applying the same equation over the interface between the phases shows that at any point on the fluid interface, 
%
\begin{equation}
\scali[1]{p}-\scali[2]{p}=\scali[1]{P}-\scali[2]{P}+(\scali[1]{\rho}-\scali[2]{\rho})\hat{\Phi}=-\scali[12]{\sigma}\kappa
\label{eq:surface_equation} ,
\end{equation}
%
where $\scali[i]{p}$, $\scali[i]{P}$ and $\scali[i]{\rho}$ are the pressure, hydrostatically adjusted pressure and density of fluid phase $i$ on each side of the interface, respectively, and
%
\begin{equation}
\kappa = \vect{\nabla} \cdot \vecti[\text{S},ij]{n}
\label{eq:kappa_ave}
\end{equation}
%
is the average signed curvature of the interface at the location \citep{brackbill92}.  As the surrounding flow is characterised by a lengthscale of $\order{\hsurround}$, and as the difference in adjusted pressures between fluid phases must be equal at any lengthscale when the system is in equilibrium, equation~(\ref{eq:surface_equation}) shows that the average curvature of the interface throughout the entire contact line region can be atmost $\order{\hsurround^{-1}}$.

However, the average curvature of a surface can be composed of two larger magnitude curvatures that are evaluated along two orthogonal surface lines and have opposing signs.  The maximum values that these two curvatures can have are known as the principal curvatures.

Far away from the three phase contact line $\hsurround$ represents the only (and hence minimum) lengthscale of the interface geometry.  Hence the principal curvatures here will both be $\order{\hsurround^{-1}}$.  Near the contact line the situation is different however.  Here, given that the fluid interface is stationary, the local angle between the fluid interface and solid surface must be equal to Young's equilibrium angle\footnote{This statement implicitly assumes that on lengthscales less than $\hrough$ the surface of the solid is smooth and displays no contact angle hysteresis.}.  In terms of the surface normals this implies
%
\begin{equation}
\vecti[{\text{S},12}]{n}\cdot\vect[w]{n}=\cos(\thetae)
\label{eq:youngs_bc} ,
\end{equation}
%
where $\vecti[{\text{S},12}]{n}$ is the unit normal to the fluid interface at a point on the three phase contact line, $\vect[w]{n}$ is the outwardly directed wall normal at the same contact point and $\thetae$ is the equilibrium angle.  Defining $\vect[2]{t}$ to be a unit vector that is tangent to the intersection of the fluid interface and wall at the contact point, and $\vecti[3]{t}=\vect[w]{n}\cross\vecti[2]{t}$ as a unit vector which is orthogonal to both $\vect[w]{n}$ and $\vecti[2]{t}$ and also lies tangential to the wall at the contact point, application of equations~(\ref{eq:kappa_ave}) and (\ref{eq:youngs_bc}) show that the curvature of the fluid interface at the three phase contact line can be expressed as
%
\begin{equation}
\scal[w]{\kappa} = -\cos(\thetae) \vect{\nabla} \cdot \vect[w]{n} + \sin(\thetae) \vect{\nabla} \cdot \vecti[3]{t} .
\label{eq:kappa_local}
\end{equation}
%
As the wall orientation vectors $\vect[w]{n}$ and $\vecti[3]{t}$ vary over the lengthscale of the surface roughness $\hrough$, equation~(\ref{eq:kappa_local}) shows that local to the three phase contact line, the magnitude of the principal curvatures of the fluid interface are $\order{\hrough^{-1}}$.

Using this curvature information we can build up a qualitative picture of the topology of the fluid interface when it is in equilibrium.  Far from the solid, that is at distances from the contact line of $\order{\rcv}$ or larger, both the principal and average curvatures of the interface are at most $\order{\hsurround^{-1}}$.  Thus, on lengthscales of order $\order{\hsurround}$ or lower the fluid interface appears flat at these locations.  Moving closer towards the solid, the average curvature remains low, but the principal curvatures increase.  Indeed, within a distance from the contact line of $\order{\hrough}$ or less, the principal curvatures will have magnitudes of $\order{\hrough^{-1}}$.  However, as the average curvature will still be low, these principal curvatures will have opposing signs.  Hence, local to the solid the topology of the fluid interface will be composed of multiple `saddle' structures, each of which will have dimensions of the size $\order{\hrough}$.


\newpage


%Under these conditions the fluid interface will also be moving slowly, and hence will effecmoves at the local velocity at its location, when local material velocities are small the fluid interface velocities are also small.  We refer to the times when the material velocities within the control volume are small (that is, approach zero) as equilibrium times.

%be $\order{\vcv}$ (or smaller) --- that is, very small.

%Formally, defining $\vect{v}$ as the local material velocity measured relative to the moving coordinates $(\vecti[1]{e},\vecti[2]{e},\vecti[3]{e})$ then for the majority of the time $\abs{\vect{v}}=\order{\vcv}$ within the control volume.

%small and consequently, the fluid interface will be in equilibrium.  This has three implications for the rough surface interface dynamics:


%As we are interested in contact angle behaviour in the limit of a slowly moving contact line, for the \emph{majority of the time} that the control volume is advancing over the solid the local velocities within the control volume must be small and consequently, the fluid interface will be in equilibrium.  This has three implications for the rough surface interface dynamics:
%
%\begin{enumerate}
%%
%\item  When the local fluid velocities are small momentum equation~(\ref{eq:momentum}) shows that fluid pressures within each phase are uniform.
%%
%\item  When the interface is in equilibrium the pressures on either side of the interface are related via
%%
%\begin{equation}
%\scali[1]{p}-\scali[2]{p}=-\scali[12]{\sigma}\kappa=-\scali[12]{\sigma}\left ( \scali[1]{\kappa} + \scali[2]{\kappa} \right )
%\label{eq:surface_equation} ,
%\end{equation}
%%
%where $\scali[1]{p}$ and $\scali[2]{p}$ are the pressures within phases $1$ and $2$, respectively, $\kappa$ is the average local interface curvature, and $\scali[1]{\kappa}$ and $\scali[1]{\kappa}$ are the principal signed local curvatures of the interface \citep{brackbill92} \footnote{This can also be shown by applying equation~(\ref{eq:momentum}) across the fluid interface assuming that $\order{\vect{v}}\rightarrow0$}.
%%
%\item  For the fluid interface to be in equilibrium the local contact angle at the three phase contact line must be equal to the Youngs eqilibrium angle, $\thetae$.  This statement implicitly assumes that on lengthscales less than $\hrough$ the surface of the solid is smooth and consequently displays no contact angle hysteresis.  In terms of the surface normals this relationship is
%%
%\begin{equation}
%\vecti[{\text{S},12}]{n}\cdot\vect[W]{n}=\cos(\thetae)
%\label{eq:youngs_bc} ,
%\end{equation}
%%
%where $\vecti[{\text{S},12}]{n}$ is the unit normal to the fluid interface at the three phase contact line, and $\vect[W]{n}$ is the outwardly directed wall normal at the same point.
%%
%\end{enumerate}
%
%Equations~(\ref{eq:surface_equation}) and (\ref{eq:youngs_bc}) infer some additional information about the geometry of the fluid interface when it is in equilibrium.  Noting that the macroscopic flow occurs on a lengthscale of $\order{\hsurround}$ (for example, a droplet of radius $\hsurround$ that sits on a solid surface), in an order of magnitude sense equation~(\ref{eq:surface_equation}) shows that when the system is in equilibrium the total interface curvature is constant (as $\scali[1]{p}$, $\scali[2]{p}$ and $\scali[12]{\sigma}$ are all constant) and given by
%%
%\begin{equation}
%\kappa=-\frac{\scali[1]{p}-\scali[2]{p}}{\scali[12]{\sigma}}=\order{\frac{1}{\hsurround}}
%%\kappa=\order{\hsurround^{-1}}
%\label{eq:macroscopic_pressure_difference} .
%\end{equation}
%%
%On the scale of the roughness however, equation~(\ref{eq:youngs_bc}) shows that the interface orientation changes over a lengthscale of $\order{\hrough}$ near the three phase contact line (the lengthscale over which $\vect[W]{n}$ changes), and hence at least one of the principal curvatures within the control volume will be $\order{1/\hrough}$.  Recalling the separation of lengthscales equation~(\ref{eq:lengthscales}), equations~(\ref{eq:surface_equation}) and (\ref{eq:macroscopic_pressure_difference}) combine to show that near the three phase contact line the average curvature of the interface can be composed of two principal curvatures, $\scali[1]{\kappa}$ and $\scali[1]{\kappa}$, whose magnitudes and signs are related by
%%
%\begin{equation}
%\scali[1]{\kappa}\approx-\scali[2]{\kappa}=\order{\frac{1}{\hrough}} .
%\end{equation}
%%
%Hence, within the control volume the geometry of the fluid interface will be flat on the lengthscale of the control volume, except near the three phase contact line where it will vary over a lengthscale of $\order{\hrough}$.
%
%\vspace{5cm}

\begin{equation}
\tau=\order{\frac{\Xcv}{\vcv}}
\label{eq:tau_mag}
\end{equation}

\begin{equation}
\abs{\vect{v}}=\begin{cases}
  \order{\vcv} & \text{for $\abs{\vect{r}}>\order{\hrough}$ and entire period $\tau$},\\
  \order{\vcv} & \text{for $\abs{\vect{r}}<\order{\hrough}$ and duration of $\scal[eq]{\tau}$ during $\tau$},\\
  \order{\vcap} & \text{for $\abs{\vect{r}}<\order{\hrough}$ and duration of $\taucap$ during $\tau$}.
\end{cases}
\label{eq:velocity_mag}
\end{equation}

\begin{equation}
\scal[eq]{\tau}=\order{\tau} \quad \text{and} \quad \taucap=\order{\frac{\Xcv}{\vcap}}%=\order{\frac{\vcv}{\vcap}\tau} 
\label{eq:cap_time}
\end{equation}

\begin{equation}
\vcap=\min \left [ \order{\frac{\sigma}{\mu}} , \order{\sqrt{\frac{\sigma}{\rho\hrough}}} \right ] \quad \text{where $\sigma=\order{\scali[ij]{\sigma}}$ for all $i<j$}
\label{eq:cap_velocity}
\end{equation}

%\newpage

\subsection{Performing the order of magnitude analysis on the mechanical energy balance}

In this section we apply the multiphase mechanical energy balance to the control volume as it advances across the surface of the solid, from $\scal[cv]{x}=0$ at $t=0$ to $\scal[cv]{x}=\Xcv$ at $t=\tau$.


\input{term_table}

\begin{equation}
E(t) = \int_{\scal[cv]{V}} \left ( \frac{1}{2}\rho v^2 + \rho \hat{\Phi} \right ) dV + 
\sum_{i<j} \scali[ij]{\sigma}\scali[ij]{A}
\label{eq:e_def}
\end{equation}

\begin{equation}
\scali[1]{T}=\scali[2]{T}+\scali[3]{T}+\scali[4]{T}+\scali[5]{T}+\scali[6]{T}+\scali[7]{T}
\label{eq:term_sum}
\end{equation}

%  Specifically, if $\vect{v}$ is the local material velocity relative to the control volume axis ($\vecti[1]{e},\vecti[2]{e},\vecti[3]{e}$), then $\order{\vect{v}}=\vcv\rightarrow0$ when the interface is in equilibrium.
%
%  Hence, for conditions within the control volume to be in equilibrium both equations~(\ref{eq:surface_equation}) and (\ref{eq:youngs_bc}) must be simultaneously satisfied.
%
%Effectively this equation specifies the geometry of the 
%
%of the within it must be small.    It also shows that when fluid velocities are small the pressures on either side of the fluid interface will be related via
%
%That the solid surface is rough has a number of implications for the dynamics of the fluid interface.
%
%As we are interested in contact angle behaviour in the limit of a slowly moving contact line, for the \emph{majority of the time} that the control volume is advancing over the solid the velocities within it must be small.  Specifically, if $\vect{v}$ is the local material velocity relative to the control volume axis ($\vecti[1]{e},\vecti[2]{e},\vecti[3]{e}$), then $\order{\vect{v}}=\vcv\rightarrow0$ for most of the time.  Applying this assumption to momentum equation~(\ref{eq:momentum}) shows that for the majority of the time the fluid pressures within each phase within the control volume will be uniform.  It also shows that when fluid velocities are small the pressures on either side of the fluid interface will be related via
%%
%\begin{equation}
%\scali[1]{p}-\scali[2]{p}=-\scali[12]{\sigma}\kappa=-\scali[12]{\sigma}\left ( \frac{1}{\scali[1]{R}} + \frac{1}{\scali[2]{R}} \right )
%%\label{eq:surface_equation} ,
%\end{equation}
%%
%where $\scali[1]{p}$ and $\scali[2]{p}$ are the pressures within phases $1$ and $2$, respectively, $\kappa$ is the average local interface curvature, and $\scali[1]{R}$ and $\scali[2]{R}$ are the pricipal signed local radii of the interface \citep{brackbill92}.  
%
%Equation~(\ref{eq:surface_equation}) specifies conditions that must be satisfied along the fluid interface for the fluid velocities to be small, however it does not must be satisfied everywhere along the fluid interface for velocities within the control volume to be small.  However for 
%
%Hence, for the fluid interface to be in equilibrium equation~(\ref{eq:surface_equation}) must be satisfied at all interface locations within the control volume.
%
%For the local three phase contact line to be in equilibrium the local contact angle between the fluid interface and the wall will be equal to the Youngs eqilibrium angle, $\thetae$ (measured through phase $1$).  In terms of the local interface surface normal $\vecti[{\text{S},12}]{n}$ and local outwardly directed wall normal $\vect[W]{n}$ this relationship is 
%%
%\begin{equation}
%\vecti[{\text{S},12}]{n}\cdot\vect[W]{n}=\cos(\thetae)
%\label{eq:youngs_bc} .
%\end{equation}
%%
%Note that this relationship implicitly assumes that on lengthscales less than $\hrough$ the surface of the solid is smooth and displays no contact angle hysteresis.  Hence, for conditions within the control volume to be in equilibrium both equations~(\ref{eq:surface_equation}) and (\ref{eq:youngs_bc}) must be simultaneously satisfied.
%
%Equation~(\ref{eq:surface_equation}) can be applied on both the lengthscale of the macroscopic flow, and on the lengthscale of the surface roughness.  On the macroscopic lengthscale the curvature of the surface will be $\order{\hrough^{-1}}$, so that $\scali[1]{p}-\scali[2]{p}=\order{\scali[12]{\sigma}/\hrough}$.  On the 
%
%That the surface of the solid is rough has two main implications in the context of contact line behaviour.
%
%The first is that the .  This has two implications for the contact angle behaviour:dual contact line speed, and microdroplet formation and destruction.
%
%\subsection{Contact line behaviour}
%
%On a rough surface, for the fluid interface to be in equilibrium two equations must be satisfied.  Firstly, 
%
%Laplace equation.  Boundary conditions.
%
%Firstly, as the fluid interface advances over the solid there will be some regions on the solid surface where the three-phase contact line cannot be in equilibrium.  In these regions the geometry of the fluid interface and solid surface is such that the local contact angle at the three phase contact line cannot equal the Youngs equilibrium angle.  More specifically, there are some locations of the three phase contact line at which the equility
%%
%\begin{equation}
%\vect[S]{n}\cdot\vect[W]{n}= \cos(\pi-\thetae)
%\end{equation}
%%
%cannot be achieved without the three phase contact line advancing.  Here $\vect[S]{n}$ and is the unit normal to the fluid interface at the three phase contact point directed into phase \circleme{1}, $\vect[W]{n}$ is the unit normal to the solid surface (wall) at the three phase contact point directed away from the solid, and $\thetae$ is the equilibrium contact angle for the combination of fluids and solid.
%
%
%
%If local equilibrium of the three phase contact line cannot be achieved, then capillary forces will rapidly move the contact line over the solid surface until a position at which equation (\ref{eq:local_equilibrium}) can be satisfied is found.  Hence, a primary implication of surface roughness is that three phase contact line will advance over the solid at two different speeds - one that is determine
%
%there will be occasions when the three phase contact line moves rapidly over the solid, even in the limit of infinitely slowly advancing fluid interface (that is, small $\vcv$).  We refer to these occasions as interface `snaps', in reference to the work of (REF).
%
%The second implication of the roughness is that small discrete packets may exist within the surface undulations.  We refer to these packets as `microdroplets'.  Microdroplets can form when fluid of one phase becomes trapped between an advancing fluid interface (that is, fluid of another phase) and roughness peaks on the solid.  Other formation mechanisms are possible, such as condensation and evaporation, however these will not be considered in this study.  Microdroplets will be destroyed when interfacial contact is made with a bulk volume of the same fluid type, and coalescence occurs.  Again, other microdroplet destruction mechanisms are possible, especially mass transfer based, however we will not consider these here.
%
%Figure \ref{fig:three_phase_micro} shows an example system where microdroplets occur on both sides of the fluid interface.  The microdroplets of phase \circleme{2} may have formed as fluid became trapped between the fluid interface and peaks of the surface undulations phase \circleme{2} advanced over the solid.  The microdroplets of phase \circleme{1} on the right of the fluid interface and under the bulk of phase \circleme{2}, which may have formed as phase \circleme{2} fluid had advanced over the solid to the left at some previous time, may recombine with the bulk of phase \circleme{1} as the interface advances over their location.  Alternatively they may stay at the base of any roughness cavities as the interface passes over (although not shown in figure \ref{fig:three_phase_micro}) forming as microdroplets of phase \circleme{1} fluid within microdroplets of phase \circleme{2} fluid.
%
%  The implications of these assumptions are discussed more fully in section \ref{sec:discuss}.

%\subsection{Control Volume Definition}



==> nomenclature.tex <==
\section{Nomenclature}

%The notation used is largely based on that used by \citet{bird02}.

\begin{supertabular}{lp{10cm}}
%Nomenclature & Definition \\ \hline
%
\multicolumn{2}{l}{\em{Arabic:}}\\
$\scali[ij]{A}$ & area of $ij$ interface type\\
$\scali[ij]{\rightarea}$ & area of $ij$ interface type entering the control volume from the right\\
$\scali[ij]{\leftarea}$ & area of $ij$ interface type leaving the control volume on the left\\
$\Acv$ & projected area of solid surface swept by CV over advance duration\\
$\widehat{\Delta \Aij}_k$ & change in interfacial area $ij$ during dissipation period $k$\\
$D$ & total energy dissipation occurring during advance\\
$\vecti[k]{e}$ & coordinate unit vector in direction $k$\\
$\vect{g}$ & gravity vector\\
$\hrough$ & lengthscale of solid surface roughness\\
$\hroughcrit$ & lengthscale of solid surface roughness that delimits viscous and inertial fluid flow regimes\\
$\hsurround$ & lengthscale of surround flow\\
$\hmol$ & lengthscale of molecular or non-continuum effects within the fluid\\
$\tens{I}$ & identity tensor\\
$\lcv$ & length of CV\\
$\ncv$ & outward normal to surface of CV\\
$\nSij$ & unit normal vector of $ij$ interface type, directed into phase $i$\\
$m$ & number of material phases present within control volume\\
$p$ & pressure\\
$p_0$ & reference pressure\\
$\dsp$ & pressure within the fluid during a dissipation period\\
$\eqp$ & pressure within the fluid during an equilibrium period\\
$\rcv$ & radius of CV\\
$\rcap$ & distance to centre of dissipation event\\
$\rcvgrav$ & capillary length\\
$\rcvmax$ & maximum applicable CV size\\
$\Scv$ & surface of CV\\
$\Scvcir$ & circumferential surface of CV\\
$\Scvend$ & end surface of CV\\
$\Scvbr$ & circumferential surface of CV at the bottom right containing compound solid interfaces\\
$\Scvbl$ & circumferential surface of CV at the bottom left containing compound solid interfaces\\
$\Scvtop$ & circumferential surface of CV at the top containing interface type $12$\\
$\Scvfluid$ & surface of CV within fluid phases\\
$t$ & time\\
$\dstk$ & start of dissipation period $k$\\
$\eqtk$ & start of equilibrium period $k$\\
$\dsDtk$ & duration of dissipation period $k$\\
$\eqDtk$ & duration of equilibrium period $k$\\
$\totT_i$ & energy term $i$ corresponding to total analysis period\\
$\dsT_{i,k}$ & energy term $i$ corresponding to dissipation period $k$\\
$\eqT_{i,k}$ & energy term $i$ corresponding to equilibrium period $k$\\
$V$ & volume\\
$\Vcv$ & volume of CV\\
$\Vcvfluid$ & volume of CV containing fluid phases\\
$\leftV$ & volume swept by $\Scvbl$ over advance duration\\
$\rightV$ & volume swept by $\Scvbr$ over advance duration\\
$\vect{v}$ & velocity\\
$\vcap$ & speed of fluid movement during dissipation events\\
$\vcv$ & speed of control volume advance\\
$\vvcv$ & velocity of control volume advance\\
$\veqv$ & velocity of fluids during equilibrium periods\\
$\vdsv$ & velocity of fluids during dissipation periods\\
$\eqnablav$ & velocity gradient within fluids during equilibrium periods\\
$\dsnablav$ & velocity gradient within fluids during dissipation periods\\
%$\vcvke$ & \\
%$\vcvvis$ & \\
%$\vcvcap$ & \\
%$\vcvkep$ & \\
%$\vcvvisp$ & \\
%$\vcvcapp$ & \\
$\Xcv$ & distance travelled by CV during total analysis period\\
$\xcv$ & distance from start of CV travel\\
$\xcap$ & location of dissipation event\\
$\vecti[\mathrm{s},ij]{x}$ & location of $ij$ interface type \\
%
\\ \multicolumn{2}{l}{\em{Greek:}} \\
$\delta$ & one dimensional Dirac delta function \\
$\deltaSij$ & surface delta function for $ij$ interface type\\
$\dsDeltasigma$ & sum of change in surface energies occurring over all dissipation events\\
$\scali[\mathrm{S},ij]{\delta}$ & surface delta function for $ij$ interface type \\
$\mu$ & viscosity\\
%$\scali[ij]{\delta}$ & Kronecker delta function \citep[p812]{bird02} \\
$\hat{\Phi}$ & gravitational potential function\\
$\rho$ & density\\
$\sigma$ & energy per unit area (interfacial tension)\\
$\sigmaij$ & energy per unit area (interfacial tension) of $ij$ interface (between phases $i$ and $j$)\\
$\rightsigma$ & compound energy per unit area solid surface entering the CV from the right and under phase \circleme{2}\\
$\leftsigma$ & compound energy per unit area solid surface leaving the CV on the left and under phase \circleme{1}\\
$\sum_{i<j}$ &  sum taken over all interface types ($=\sum_{j=1}\sum_{i=1}^{j-1}$)\\
$\tens[M]{T}$ & material stress tensor\\
$\tens[S]{T}$ & interfacial stress tensor\\
$\taucap$ & total duration of dissipation events occurring during CV advance\\
$\thetaa$ & macroscopic advancing angle of phase \circleme{1} in phase \circleme{2}\\
$\thetar$ & macroscopic receding angle of phase \circleme{1} in phase \circleme{2}\\
$\thetae$ & equilibrium angle of phase \circleme{1} in phase \circleme{2}\\
%
%\\ \multicolumn{2}{l}{\em{Subscripts:}} \\
%cv & control volume \\
%
%\\ \multicolumn{2}{l}{\em{Superscripts:}} \\
\end{supertabular}


==> old_paper.tex <==










\section{Introduction}

\subsection{Lit review:}

\subsubsection{Theory:}

Early works, looking at energy change with interface movement
\citet{wenzel36} --- both phases completely wetting, but interface area increases
\citet{cassie44} --- builds on wenzel, rough surface, but one phase does not wet surface --- applied to porous surfaces to good effect --- may also describe energy balance at contact line with superhydrophobic surfaces.

\citet{johnson64}

\citet{long05} --- looks at energy change as droplet free energy changes as droplet moves over individual surface oscillations --- These studies predict that contact angle hysteresis should decrease as size of oscillations decreases, as energy barriers to movement become smaller.  These trends are not seen experimentally --- see eg \citet{brandon03}

Similar, related, vein: contact line halted by individual surface topology --- ie, force balance on contact line on uneven surface \citet{shuttleworth48} --- does not match experimental observation, eg, \citet{miller96} study referred to in \citet{long05} study --- different surface `angles' in different directions --- what physical basis???

\begin{figure}[h]
\centering%
\subfigure[\label{fig:dettre64b_fig1}]{\includegraphics[keepaspectratio,width=0.48\textwidth]{./figures/angle_scans/dettre64b_fig1.png}}%
\subfigure[\label{fig:dettre64b_fig2}]{\includegraphics[keepaspectratio,width=0.48\textwidth]{./figures/angle_scans/dettre64b_fig2.png}}%
\caption{Water contact angles on TFE-methanol telomer wax surface as a function of roughness (a) and photomicrographs of the same surfaces (b) \citep[taken from][]{dettre64b}.}%
\label{fig:dettre64b_fig12}%
\end{figure}

\subsubsection{Experiments:}

Some do not appreciate difference between advancing on wet and dry surfaces, description somewhat vague.
Limited quantitative data on nature of surface roughness useful for hysteresis prediction, however, some studies give qualitiative description of surface (AFM,ESM etc).
Studies may be complicated by adsorbtion and chemical effects.

\citet{miller96}
\citet{lam01}

\citet{muller01} grew well defined `nanopyramids' on surface, and found that \emph{....contact-angle hysteresis can partly be explained by the barrier effect, which gives rise to symmetric hysteresis, and the capillary effect, which leads to a contact angle reduction, (but) another phenomenon must exist to describe the hysteresis shown in figure 3...} (ALSO, QUESTION THEN, WHAT SCALES DOES THEORY GO DOWN TO?)

%Purpose:  To use a heuristic model of nanobubble formation to simulate contact angle hysteresis.

\subsection{Purpose}

The purpose of this paper is to explain the phenomenon of contact angle hysteresis in terms of microbubble formation and relaxation.   In this context `microbubble' describes any small packet of fluid which exists within the depressions of the rough solid surface, but is bounded above by another fluid with which it is immiscible.  After formulating the problem in general terms, we propose a simple model for the kinetics of a bubble which is formed and relaxes on a saw tooth surface.  We use this model to find advancing and receding angles on both dry and wet surfaces in terms of the `Youngs' equilibrium angle and two solid roughness parameters.  Predictions from the model reproduce some fundamental experimental observations, reinforcing the postulate that rough solid contact angle hysteresis is a macroscopic manifestation of microbubble kinetics.



%In this paper we explain the phenomenon of rough surface contact angle hysteresis using a model of rough surface nanobubble formation and relaxation. 

%are trapped in the surface roughness  kinetics formation s which form and then relax in the depressions in the solid durface.   formation and relaxation on the solid 

\section{Model Formulation}

%In this section we describe in general terms how microbubbles form and relax as a fluid interface sweeps over a rough solid surface.  This is then used to explain, using an energy balance, contact angle hysteresis in terms of microbubble kinetics.  We then develop a specific model of bubble behaviour on a saw tooth surface, and detail the numerical procedure used to generate curves of advancing and receding angles for this model surface in terms of the Youngs equilibrium angle, and two solid surface roughness parameters.

\subsection{Microbubble Behaviour}

Figure \ref{fig:energy_balance}(a) shows the physical system that we analyse.  It consists of two phases, labelled $1$ and $2$, which are bounded below by a rough solid.  The phases may be either liquid or gas, but are immiscible with each other.  The main interface between the phases, line $AB$ in the figure, is moving at a vanishingly slow velocity $v$ to the right so that phase $1$ is advancing across the solid, and phase $2$ receding.  On the length scale of this figure, the angle that the interface is orientated at far away from the surface undulations is $\scal[m]{\theta}$, measured through phase $1$.  This angle is the advancing angle for phase $1$, being defined as the minimum interface angle that \emph{just} produces movement of the interface to the right, or equivalently, as the maximum angle at which the interface \emph{just} remains stationary --- under either definition $v$ will be vanishingly slow, or in order of magnitude terms, $\order{v}=0$.

\begin{figure}[htbp]
\centering
\resizebox{\textwidth}{!}{\input{triple_line_balance.pdf_t}} % fig from xfig that includes latex text
\label{fig:triple_line_balance}
\caption{Frame (a) shows the region surrounding the control volume (cv) and contact line on a macroscopic scale, while frame (b) shows the same region on the scale of the microbubbles present within the cavities of the solid surface.  The symbols \protect\circleme{1}, \protect\circleme{2}, and \protect\circleme{S}, indicate regions of phase $1$ fluid, phase $2$ fluid, and solid, respectively.}
\end{figure}

Figure \ref{fig:triple_line_balance}(b) shows how the system may be related to the surrounding flow.  In this example a droplet of phase $1$ fluid is advancing over a solid while the surrounding phase $2$ fluid is receding.  The length scale of the surrounding flow is $\hsurround$, in this case taken to be the local radius of the phase $1$ droplet.  On the length scale of the surrounding flow $\scal[m]{\theta}$ is the angle at which the interface of the droplet intersects with the solid.  Thus, we can formally define the measured advancing interface angle to be
%
\begin{equation}
\scal[m]{\theta}=\theta(\epsilon) \mbox{,} \label{eq:thetam}
\end{equation}
%
where $\theta(l)$ is the angle of the interface at a distance $l$ from point $B$, and $\epsilon$ is a small distance satisfying $\hrough\ll\epsilon\ll\hsurround$.  Note that although the problem is formulated in terms of the advancing angle of phase $1$, the receding angle of phase $1$ may be calculated by interchanging phase properties and calculating the advancing angle of phase $2$.

Microbubbles exist within the roughness cavities of the solid on either side of the interface $AB$ (see figure \ref{fig:triple_line_balance}(a)).  To the right of point $B$, these bubbles are packets of phase $1$ fluid that are bounded above by phase $2$ fluid.  To the left of point $B$, the bubbles are packets of phase $2$ fluid, bounded above by phase $1$ fluid.

The origin of the phase $1$ bubbles to the right of $B$ is immaterial at this stage of the analysis, however we assume that they have existed within the solid cavities for long enough that molecular vibration has allowed their interfacial areas to change, and in so doing, the total energy of the solid interface to the right of point $B$ has minimised --- these bubbles are in a `relaxed' state.  As the interface $AB$ moves to the right and intersects with these bubbles, the bubbles collapse and the fluid that they contain combines with the majority of phase $1$ fluid to the left of $B$.  Associated with each bubble collapse is the generation of significant local fluid velocities.  The majority of the kinetic energy represented this local flows is converted to heat via viscous dissipation.

The microbubbles to the left of point $B$, that is the bubbles of phase $2$ fluid bounded above by phase $1$ fluid, are formed as the interface $AB$ sweeps to the right, trapping packets of phase $2$ fluid between adjacent roughness peaks of the solid and the bulk of phase $1$ as it proceeds.  At the moment these bubbles are formed, that is, at the moment each bubble separates from the bulk of the phase $2$ fluid, its upper interface is stretched in the direction of the main interface $AB$.  Thus, these bubbles are in a higher energy state at the moment they are created than the relaxed bubbles to the right of point $B$.

After a period of time, the interfaces of the stretched phase $2$ bubbles to the right of point $B$ move as a result of molecular vibrations, so that the total interfacial energy of the solid interface in this region decreases and the bubbles approach a relaxed energy state.  The interfacial energy that is lost by the solid surface region as these bubbles relax is converted to heat via the viscous motion of the surrounding fluid.  If another fluid interface traverses this solid region and consumes these phase $2$ bubbles, or alternatively if the direction in which the interface $AB$ moves is reversed and the phase $2$ bubbles are recombined with the bulk of the phase $2$ fluid again, the bubbles will be in a relaxed state prior to consumption.  This is consistent with the phase $1$ bubbles which exist to the right of the interface $AB$ in figure \ref{fig:energy_balance} also being relaxed prior to consumption.

%Thus, if another fluid interface traverses this region and collects these phase $2$ bubbles, the system will be equivalent to that described above, but with the relaxed phase $2$ bubbles now represented as phase $1$ , the Thus, if the direction of movement of the interface $AB$ is reversed and the bubbles recombine with the bulk of the phase $2$ fluid, the phase $2$ bubbles these bubbles will be in a relaxed energy state.

CONSIDERING INCOMPRESSIBLE BUBBLES ONLY RIGHT NOW, MORE ON THIS IN DISCUSSION

\subsection{Energy Balance}


\begin{equation}
\frac{dE}{dt} = \scal[int]{v}\scal[relax]{\hat{\sigma}} - \scal[int]{v}\scal[relax]{\bar{\sigma}} - \scal[int]{v}\scal[12]{\sigma}\cos\scal{\theta} + \scal[2]{Q}(\scal[2]{P}-\scal[2]{\bar{P}}) + \scal[1]{Q}(\scal[1]{\hat{P}}-\scal[1]{P}) - D
\label{eq:energy}
\end{equation}

\begin{equation}
\scal[1]{Q}=\scal[int]{v}\scal[1]{\hat{V}} \mbox{ and } \scal[2]{Q}=\scal[int]{v}\scal[2]{\bar{V}} 
\label{eq:flowrates}
\end{equation}

\begin{equation}
\order{\scal[1]{P}}=\order{\scal[2]{P}}=\order{\frac{\scal[12]{\sigma}}{\hsurround}}\ll\order{\frac{\scal[12]{\sigma}}{\hrough}}=\order{\scal[1]{\hat{P}}}=\order{\scal[2]{\bar{P}}}
\label{eq:pressure}
\end{equation}

\begin{equation}
D=\int_V \tens{\tau} : \vect{\nabla}\vect{v} dV = \scal[c]{D} + \scal[d]{D}
\label{eq:dissipation}
\end{equation}

\begin{equation}
\order{\scal[c]{D}} = \order{\mu \scal[int]{v}^2} \rightarrow 0
\label{eq:dissipation_c}
\end{equation}

\begin{equation}
\scal[d]{D} = \left[ \scal[contact]{\hat{\Phi}} + \scal[relax]{\hat{\Phi}} + \scal[adjust]{\hat{\Phi}} \right] \scal[int]{v}
\label{eq:dissipation_d}
\end{equation}

\begin{equation}
\scal[contact]{\hat{\Phi}} = \left[ \scal[relax]{\hat{\sigma}}(\scal[1]{\hat{V}}) - \scal[relax]{\hat{\sigma}}(0) + \scal[1]{\hat{P}}\scal[1]{\hat{V}}  \right] \scal[contact]{c}
\label{eq:dissipation_contact}
\end{equation}

\begin{equation}
\scal[relax]{\bar{\Phi}} = \left[ \scal[stretch]{\bar{\sigma}}(\scal[2]{\bar{V}}) - \scal[relax]{\bar{\sigma}}(\scal[2]{\bar{V}}) - \scal[2]{\bar{P}}\scal[2]{\bar{V}}  \right] \scal[relax]{c}
\label{eq:dissipation_relax}
\end{equation}

\begin{equation}
\scal[adjust]{\Phi} \approx 0
\label{eq:dissipation_adjust}
\end{equation}

\begin{equation}
c = \scal[relax]{c} = \scal[contact]{c}
\label{eq:c}
\end{equation}

\begin{eqnarray}
f(\theta) &= &(1-c)\scal[relax]{\bar{\sigma}}(\scal[2]{\bar{V}}) + c \scal[stretch]{\bar{\sigma}}(\scal[2]{\bar{V}}) + (1-c)\scal[2]{\bar{P}}\scal[2]{\bar{V}} \nonumber \\
& - & (1-c)\scal[relax]{\hat{\sigma}}(\scal[1]{\hat{V}}) - c\scal[relax]{\hat{\sigma}}(0) - (1-c)\scal[1]{\hat{P}}\scal[1]{\hat{V}} \nonumber \\
& + & \cos\theta
\label{eq:f}
\end{eqnarray}

Require for advancing angle:

\begin{equation}
f(\scal[m]{\theta}) = 0 \mbox{ and } \frac{\partial f}{\partial \theta} ( \scal[m]{\theta} ) < 0
\label{eq:f_conditions}
\end{equation}

CLEANUP DIMENSIONLESS NOTATION

V. ROUGH FROM HERE ON

In the previous section we described our basic postulate as to how bubbles form and then relax as a fluid interface sweeps over a rough solid surface.  To determine how this bubble behaviour influences contact angle hysteresis, we perform an energy balance on the interface region surrounding the contact line between the two fluid phases and solid surface.

%Figure \ref{fig:energy_balance} shows the control volume that we use.  The volume has a height $h$ above the mean solid surface height and traverses a significant number of solid surface undulations.  As described above, bubbles of phase $1$ fluid to the right of point $B$ are consumed as the interface moves forward, while bubbles of phase $2$ fluid to the left of point $B$ are generated.  As the bubbles of phase $2$ fluid are completely separate from the main fluid interface once they have been generated, the energy they subsequently dissipate by moving from the stretched to relaxed state does not influence the resulting advancing angle.  Thus, for the purposes of predicting the advancing angle we assume that the phase $2$ bubbles to the left of point $B$ remain in their stretched state while within the control volume.

%Consistent with the premise that the interface $AB$ is energetically on the border between slowly moving forward and remaining stationary, velocities within each fluid phase are assumed to be vanishingly small so that all viscous and inertial forces within each fluid are zero.  This assumption, combined with the neglect of body forces, implies that the pressure within each phase is constant.  We define $\scal[1]{P}$ and $\scal[2]{P}$ to be the pressures within phases $1$ and $2$, respectively, and the flowrates of phases $1$ and $2$ into the control volume to be $\scal[1]{Q}$ and $\scal[2]{Q}$, respectively.




Defining the total energy per unit projected area of the solid interface to the right of point $B$ as
%
\begin{equation}
\bar{\sigma} = \frac{ \scal[12]{\sigma}\scal[12]{\bar{A}} + \scal[1s]{\sigma}\scal[1s]{\bar{A}} +\scal[2s]{\sigma}\scal[2s]{\bar{A}} }{\scal[t]{A}} \mbox{,}
\label{eq:barsigma1}
\end{equation}
%
then this `relaxation' concept can be quantitatively expressed as $\scal[12]{\bar{A}}$, $\scal[1s]{\bar{A}}$ and $\scal[1s]{\bar{A}}$ changing to minimise $\bar{\sigma}$, subject to the constaint that the total volume of phase $1$ per unit projected area of solid surface to the right of point $B$, $\bar{V}$, is constant.  In the above $\scal[12]{\bar{A}}$ is the interfacial area per unit projected area of the solid between phases $1$ and $2$ that exists to the right of point $B$.  Similarly, $\scal[1s]{\bar{A}}$ and $\scal[2s]{\bar{A}}$ are the interfacial areas per unit projected area of the solid between phase $1$ and the solid, and phase $2$ and the solid, both to the right of point $B$, respectively.  Also, the total area of the solid surface per unit projected area of the surface is $\scal[t]{A}$, and $\scal[12]{\sigma}$, $\scal[1s]{\sigma}$ and $\scal[2s]{\sigma}$ are the interfacial energies of the interfaces between phases $1$ and $2$, phase $1$ and the solid, and phase $2$ and the solid, respectively.


  We note that our model presumes that individual bubbles remain in individual solid cavities as they relax.  This assumption requires that the height of the solid surface undulations, $R$, is significantly larger than the molecular free path of the molecules near the fluid interface so that the three phase contact line cannot `jump' over individual surface undulations.  Conservatively we can express this assumption as $\order{\max(\scal[1]{\lambda},\scal[2]{\lambda})/R}<<1$, where $\scal[1]{\lambda}$ and $\scal[2]{\lambda}$ are the mean free paths of molecules within phases $1$ and $2$, respectively.



%Per unit area of the solid surface, they have a volume $\bar{V}$, an interfacial area with phase $2$ of $\bar{\scal[12]{A}}$ and interfacial area of 
%These bubbles have associated with them an area with phase $2$ fluid which exists above them, $\bar{\scal[12]{A}}$, 

%`Bubbles' of phase $2$ may exist at the interface of the solid and phase $1$, as shown in the figure.  Theses bubbles are formed as the interface 


%While the interface $AB$ destroys the relaxed phase $1$ bubbles that exist on the receding solid surface as it moves to the right, it may create phase $2$ bubbles on the advancing solid surface by trapping small packets of phase $2$ fluid between the bulk of phase $1$ fluid, and individual  adjacent roughness cavities of the solid surface.

3 length scales
timescale of relaxation v interface movement

\citet{tyrrell01} --- Nanobubble existence, through to different length scales, bubbles stable within surface roughness

\pagebreak

\subsection{Microbubble Kinetics on a Sawtooth Surface}

\begin{figure}[htbp]
\centering
\resizebox{0.7\textwidth}{!}{\input{sawtooth.pdf_t}} % fig from xfig that includes latex text
\label{fig:sawtooth}
\caption{Basic geometry of model sawtooth surface.}
\end{figure}

Required from local surface model:
%
\begin{list}{$\bullet$}{}
\item Volume left on left (after sweep): $\scal[2]{\bar{V}}=\scal[2]{\bar{V}}( \theta,\thetae )$
\item Energy of relaxed bubbles on left: $\scal[relax]{\bar{\sigma}}=\scal[relax]{\bar{\sigma}}( \scal[2]{\bar{V}},\thetae )$
\item Energy of stretched bubbles on left: $\scal[stretch]{\bar{\sigma}}=\scal[stretch]{\bar{\sigma}}( \scal[2]{\bar{V}},\thetae,\theta )$
\item Energy of relaxed bubbles on right: $\scal[relax]{\hat{\sigma}}=\scal[relax]{\hat{\sigma}}( \scal[1]{\hat{V}},\thetae )$
\item Pressure within relaxed bubbles on left: $\scal[2]{\bar{P}}=\scal[2]{\bar{P}}( \scal[2]{\bar{V}},\thetae )$
\item Pressure within relaxed bubbles on right: $\scal[1]{\hat{P}}=\scal[1]{\hat{P}}( \scal[1]{\hat{V}},\thetae )$
\end{list}

CHART OF ALGEBRAIC FORMULAE

\subsubsection{Formation}
\subsubsection{Relaxation}

\section{Numerical Solution Process}

\section{Results}

\citet{sedev93} --- Basic behaviour for hydrophylic droplet --- advancing dry, receding wet, advancing wet

\begin{figure}[p]
\centering%
\includegraphics[keepaspectratio,height=\textwidth,angle=-90]{/home/daltonh/doc/contact_angles/dhcontact07/figures/sedev93/printme.pdf}%
\caption{Equilibrium $\thetae$, receding $\scal[r]{\theta}$, and wet advancing $\scal[a,wet]{\theta}$ angles and non-dimensional volume left residing in the surface as a function of dry advancing angle $\scal[a,dry]{\theta}$.  Here $R=0.3$, $\scal[w]{\lambda}=1.0$ and $c=0.9$, approximating the data from \citet{sedev93}.  INCLUDE EFFECT OF VARYING $c$.}
\end{figure}

\citet{dettre64b} --- predicts angle accurately as same liquid applied over changing surface roughness --- exp noticed air under droplet...

\begin{figure}[p]
\centering%
\includegraphics[keepaspectratio,height=\textwidth,angle=-90]{/home/daltonh/doc/contact_angles/dhcontact07/figures/dettre64b_fig1/triangle_n107_r1.3_c0.9_lambdaw/printme.pdf}%
\caption{Advancing and receding angle and non-dimensional volume left residing in the surface as a function of $1/\scal[w]{\lambda}$.  Here $\thetae=107\degrees$, $R=1.3$ and $c=0.9$, approximating the data from \citet{dettre64b}, figure 1.}
\end{figure}

\begin{figure}[p]
\centering%
\includegraphics[keepaspectratio,height=\textwidth,angle=-90]{/home/daltonh/doc/contact_angles/dhcontact07/figures/dettre64b_fig1/triangle_n104_lambdaw1_c0.9_r/printme.pdf}%
\caption{Advancing and receding angle and non-dimensional volume left residing in the surface as a function of $R$.  Here $\thetae=104\degrees$, $\scal[w]{\lambda}=1.0$ and $c=0.9$, approximating the data from \citet{dettre64b}, figure 1.}
\end{figure}

\citet{busscher84} --- behaviour as a function of $\theta_e$, same surface, hydrophobic and hydrophilic

\citet{miller96} --- options for these trends

\citet{lam01} --- NB, as droplet radius decreases, pressure inside droplet increases, changes receding contact angle by changing area of microbubbles under liquid and changing flow work

\section{Discussion}

Bigger picture:  Analysis and experimental comparison points to formation of nano-microbubbles on rough surfaces.  Or, probably more significantly and more relvantly, at least the stabilisation of microbubbles on a rough surface.  IE, once formed, with however means, they are capable of staying there.  Need to discuss pressure within bubbles a bit more, and REF William's work with measured pressure in bubbles --- supports compound curvature assumption.  For example:
%
\begin{itemize}
%
\item Several researchers have discussed the presence of nanobubbles as an explanation for observed long range attraction forces between hydrophobic surfaces \citep[][for example]{ishida00,tyrrell01,yang03a,attard03,mao04}.  It is argued that if nanobubbles are present on either surface, then when the two surfaces are brought together contact between a bubble attached to one surface and the adjacent surface will occur at a certain separation distance, causing the bubble to abruptly attach to both surface simultaneously --- so called `bridging'.  This explanation is consistent with a significant attractive force abuptly appearing between hydrophobic surfaces as they approach, and an abrupt decrease in this force at a larger separation when the surfaces are later drawn apart.  There is considerable discussion as to the orgin of these bubbles however.  While some studies suggest that nanobubbles can form spontaneously under conditions where the liquid is highly saturated with gas, the present analysis suggests that bubbles may (also) be present in roughness cavities from the time at which the surface was originally wetted (REFS).

There is also discussion as to what \emph{...the `critical size' of surface physical defects or crevices necessary for bubble formation...} is \citep{yang03a}.  If the bubbles present on the surface are formed via the contact line mechanisms examined here, then it is not the amplitude of roughness defects that is the critical parameter in determining bubble formation, but rather the local gradients of the surface (subject to $\hrough>>\lambda$).  This may explain observed differences in `hydrophobic' attaction forces between surfaces of apparently similar roughness amplitudes (REFS).
%
\item Several authors have employed the idea of a `line tension' when interpreting experimental results \citep[][eg]{yang03a}:  That is, a tension which acts along the three phase contact line.  There does not appear to be a clear physical mechanism for the existence of such a force however, certainly not on nondeformable surfaces (REFS).  The current model shows that dissipation of energy occurs when the contact line moves over a rough surface, even when $\order{\scal[int]{v}}=0$.  Experimentally, this energy loss could be interpreted as a `line tension' which has a sign which is inversely proportional to the direction of interface movement, and in the limit of a stationary interface, a magnitude of zero.  Thus, the present theory suggests a physical mechanism for the existence of `line tension'.
%
\item In experiments where a liquid jet containing air bubbles impinged upon both hydrophobic and hydrophillic surfaces, \citet{yang03b} found that at the lowest flowrates the `bubble-attachment flux' was higher than predicted by a mass transfer theory.  Amongst several explanations offered for the discrepancy was the neglect of surface roughness effects on stabilising bubble capture.
%
\end{itemize}

Much further work to consider.

\begin{itemize}
%
\item Compressibility of gas in microbubbles not considered yet:  However, effect of compression due to increase in microbubble pressure possibly not straight forward as have to make assumption re what pressure within relaxed bubble is --- have min and max limits though, IE, just the bulk pressure -> full capillary force, as assumed here.
%
\item Important to many applications which involve droplet impact and spreading (coatings, spray cooling, etc) is how the contact angles vary with the macroscopic droplet size.  Numerous experimental results show a dependence of both advancing (CHECK!) and receding angles on the macroscopic droplet radius when this radius is small \citep{lam01,lam02}.  The dependence of contact angle on macroscopic droplet size could be incorporated into the present analysis by relaxing the condition that $\hrough<<\hsurround$.  In so doing equation (\ref{eq:pressure}) would now give non zero fluid bulk pressures within the control volume, ($\order{\scal[1,2]{P}}\ne0$), and as a result, the flow work terms contained in the energy balance equation (\ref{eq:energy}) would lead to a dependence between $\scal[m]{\theta}$ and the droplet radius.  Indeed, in line with the experimental observations of \citet{lam01},.... (CHECK THAT CORRECT SIGN RESULTS!).

As a secondary affect, the dimensions of any relaxed gaseous microbubbles entering into the analysis may change with nonzero surrounding bulk pressures, producing a further dependence of contact angle on macroscopic droplet size (THINK, EXAMINE OTHER TERMS).
%
\item Have not looked at effect of dissolution of bubbles on hysteresis, however, given the energy balance is performed over a small region local to the three phase contact line, the timescale of bubble dissolution may be too long to enter into the analysis.  (COULD GET REPRESENTATIVE TIMESCALE)
%
\end{itemize}

\section{Conclusions}


\vspace*{1.5em}\noindent\textbf{Acknowledgements:}  The author would like to thank Prof. Franz Grieser and Prof. William Ducker for discussions....


\appendix

\section{Macroscopic Mechanical Energy Balance with Surface Energy}

In this section we derive a macroscopic mechanical energy balance for a moving and deforming control volume which contains a number of immiscible fluids.  The derivation is identical to that given in \citet[][p221, \S 7.8]{bird02}, except that it includes surface energy terms.

Our starting point for the derivation is a momentum equation for a mixture of immiscible fluids,
%
\begin{equation}
\frac{\partial}{\partial t}\rho\vect{v} = - \vect{\nabla} \cdot  \rho\vect{v}\vect{v} - \vect{\nabla}p - \vect{\nabla} \cdot \tens[v]{\tau} + \rho\vect{g} + \vect{\nabla} \cdot \tens[s]{\tau} 
\end{equation}
%
As the fluid properties used in this equation (e.g. density $\rho$) vary with location, the equation is valid both on the boundaries and within the volume of any of the fluids.  The effects of interfacial tension on fluid movement are captured using a surface stress tensor, defined by
%
\begin{equation}
\tens[s]{\tau}(\vect{x}) = \sum_{i<j} ( \tens{I} - \vecti[\mathrm{s},ij]{n} \vecti[\mathrm{s},ij]{n} ) \sigmaij \scal{\delta}(\vect{x}-\vecti[\mathrm{s},ij]{x})
\end{equation}
%
where $\vecti[\mathrm{s},ij]{n}$ is a unit normal between phases $i$ and $j$ which is directed into phase $i$, $\sigmaij$ is the surface energy (per unit area) of the interface between phases $i$ and $j$, $\vecti[\mathrm{s},ij]{x}$ specifies the surface location of the interface between phases $i$ and $j$, and $\delta$ is the Dirac delta function.  The Dirac delta function is defined so that the total area of the surface between phases $i$ and $j$ in volume $V$ is given by
%
\begin{equation}
\scali[ij]{A} = \int_{V} \scal{\delta}(\vect{x}-\vecti[\mathrm{s},ij]{x}) dV_{\vect{x}}
\end{equation}

\newpage



ETC



\bibliography{abbreviated,droplet,daltonh,suspend,microfluidics,cangle}
\end{document}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

NB: nanobubble = microbubble = nano/micro droplet
evidence of nanobubbles --- afm studies



==> term_table.tex <==
%\begin{table}[p]
\begin{sidewaystable}[p]
%\hspace{-1.5cm}
%\hspace*{-1.5cm}
\begin{center}
\begin{tabular}{l@{\hspace{2ex}}l@{\hspace{4ex}}l} \toprule%
%
\emph{Term} & \emph{Definition} & \emph{Order of magnitude} \\ \midrule
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{tableeqn}
\scali[1]{T}
\end{tableeqn} &
%
\begin{tableeqn}
\frac{E(t=\tau)-E(t=0)}{\scal[cv]{A}}
\end{tableeqn} &
%
\begin{tableeqn}
\order{\frac{\rho\scal[cap]{v}^2\scal[rough]{h}^2}{\scal[cv]{X}}} +
\order{\frac{\rho\scal[cv]{v}^2\scal[cv]{r}^2}{\scal[cv]{X}}} +
\order{\frac{\rho g\scal[cv]{r}^3}{\scal[cv]{X}}} +
\order{\frac{\sigma \scal[cv]{r}}{\scal[cv]{X}}}
\end{tableeqn} \\
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{tableeqn}
\scali[2]{T}
\end{tableeqn} &
%
\begin{tableeqn}
\frac{1}{\scal[cv]{A}} \int^\tau_0 \int_{\scal[cv]{S}} \vect[cv]{n} \cdot \frac{1}{2}\rho v^2 ( \vect[cv]{v} - \vect{v} ) \, dS dt
\end{tableeqn} &
%
\begin{tableeqn}
\order{\rho \scal[cv]{v}^2 \scal[cv]{r}} + 
\order{\frac{\rho\scal[cv]{v}^2\scal[rough]{h}^2}{\scal[cv]{l}}}
\end{tableeqn} \\
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{tableeqn}
\scali[3]{T}
\end{tableeqn} &
%
\begin{tableeqn}
\frac{1}{\scal[cv]{A}} \int^\tau_0 \int_{\scal[cv]{S}} \vect[cv]{n} \cdot \rho \hat{\Phi} ( \vect[cv]{v} - \vect{v} ) \, dS dt
\end{tableeqn} &
%
\begin{tableeqn}
\order{\rho \scal[cv]{r}^2 g}
\end{tableeqn} \\
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{tableeqn}
\scali[4]{T}
\end{tableeqn} &
%
\begin{tableeqn}
\frac{1}{\scal[cv]{A}} \int^\tau_0 \int_{\scal[cv]{S}} \sum_{i<j} \scali[ij]{\sigma} \scali[\text{S},ij]{\delta} ( \vect[cv]{v} - \vect{v} ) \, dS dt
\end{tableeqn} &
%
\begin{tableeqn}
\order{}
\end{tableeqn} \\
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{tableeqn}
\scali[5]{T}
\end{tableeqn} &
%
\begin{tableeqn}
\frac{1}{\scal[cv]{A}} \int^\tau_0 \int_{\scal[cv]{S}} \sum_{i<j} \scali[ij]{\sigma} \scali[\text{S},ij]{\delta} \left ( \tens{I} - \vecti[\text{S},ij]{n} \vecti[\text{S},ij]{n} \right ):\vect{v} \vect[cv]{n} \, dS dt
\end{tableeqn} &
%
\begin{tableeqn}
\order{}
\end{tableeqn} \\
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{tableeqn}
\scali[6]{T}
\end{tableeqn} &
%
\begin{tableeqn}
\frac{1}{\scal[cv]{A}} \int^\tau_0 \int_{\scal[cv]{S}} \tens[M]{T}:\vect{v} \vect[cv]{n} \, dS dt
\end{tableeqn} &
%
\begin{tableeqn}
\order{}
\end{tableeqn} \\
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{tableeqn}
\scali[7]{T}
\end{tableeqn} &
%
\begin{tableeqn}
\frac{1}{\scal[cv]{A}} \int^\tau_0 \int_{\scal[cv]{V}} \tens[M]{T}:\vect{\nabla} \vect{v} \, dV dt
\end{tableeqn} &
%
\begin{tableeqn}
\order{}
\end{tableeqn} \\
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule%
%
\end{tabular}
\end{center}
\caption{Seven terms comprise the multiphase mechanical energy balance as applied to the moving three phase contact line.  \label{tab:terms}}
%\end{table}
\end{sidewaystable}

